The Virgo O3 run and the impact of the environment

Sources of geophysical noise (such as wind, sea waves and earthquakes) or of anthropogenic noise impact ground-based gravitational-wave interferometric detectors, causing transient sensitivity worsening and gaps in data taking. During the one year-long third Observing Run (O3: from April 01, 2019 to March 27, 2020), the Virgo Collaboration collected a statistically significant dataset, used in this article to study the response of the detector to a variety of environmental conditions. We correlated environmental parameters to global detector performance, such as observation range, duty cycle and control losses. Where possible, we identified weaknesses in the detector that will be used to elaborate strategies in order to improve Virgo robustness against external disturbances for the next data taking period, O4, currently planned to start at the end of 2022. The lessons learned could also provide useful insights for the design of the next generation of ground-based interferometers.

==> definitions.tex <==
\usepackage{graphicx}
\usepackage{color}
\usepackage[table]{xcolor}
\usepackage{epsfig}
\usepackage{float}
\usepackage{multirow}
\expandafter\let\csname equation*\endcsname\relax
\expandafter\let\csname endequation*\endcsname\relax
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{tabularx,url,color}
\usepackage{hyperref}
\usepackage[T1]{fontenc}

\usepackage{lineno}
\usepackage{upgreek}

\usepackage{subfig}

\RequirePackage{xspace}

\usepackage[subfigure]{tocloft} % Notice the option, needed not to mess up with subfig

\newcommand\rednote[1]{\textcolor{red}{\bf {#1}}}
\newcommand\bluenote[1]{\textcolor{blue}{\bf {#1}}}

\newcommand{\VirgoAcronym}[3]{ \noindent {\bf #1}: {\it #2}, #3. \\}
\newcommand{\VirgoAcronymShort}[2]{ \noindent {\bf #1}: #2. \\}

\newcommand{\Reviewer}[1]{~\\ \noindent {\textcolor{purple}{\bf {Reviewer(s): #1}}} \\}
\newcommand{\Writer}[1]{~\\ \noindent {\textcolor{blue}{\bf {Writer(s): #1}}} \\}

\newenvironment{oldtext}{~\\ \color{olive}{\bf $<$OLDTEXT$>$}}{\bf $<$/OLDTEXT$>$ ~\\}

\newcommand{\bea}{\begin{eqnarray*}}
\newcommand{\eea}{\end{eqnarray*}}
\newcommand{\beao}{\begin{eqnarray}}
\newcommand{\eeao}{\end{eqnarray}}
\newcommand{\no}{\noindent}

\definecolor{lightgray}{gray}{0.9}

\endinput

